Urban Mobility Assessment Using LLMs

Understanding urban mobility patterns and analyzing how people move around cities helps improve the overall quality of life and supports the development of more livable, efficient, and sustainable urban areas. A challenging aspect of this work is the collection of mobility data by means of user tracking or travel surveys, given the associated privacy concerns, noncompliance, and high cost. This work proposes an innovative AI-based approach for synthesizing travel surveys by prompting large language models (LLMs), aiming to leverage their vast amount of relevant background knowledge and text generation capabilities. Our study evaluates the effectiveness of this approach across various U.S. metropolitan areas by comparing the results against existing survey data at different granularity levels. These levels include (i) pattern level, which compares aggregated metrics like the average number of locations traveled and travel time, (ii) trip level, which focuses on comparing trips as whole units using transition probabilities, and (iii) activity chain level, which examines the sequence of locations visited by individuals. Our work covers several proprietary and open-source LLMs, revealing that open-source base models like Llama-2, when fine-tuned on even a limited amount of actual data, can generate synthetic data that closely mimics the actual travel survey data, and as such provides an argument for using such data in mobility studies.

==> sections/inter-city-results.tex <==
\section{Holistic evaluation of the system using simulated data for multiple cities}
\label{sec:inter-city-results}

This section provides an analysis of the outputs generated by our LLM-based travel survey simulation system for all five cities to measure the overall efficacy of the simulation system. 
In this section, we limit the models of choices to Llama-2 base, Gemini-pro, GPT-4, and Llama-2-trained-x-infer models.

Table~\ref{tab:inter_loc_travel_time_chain_analysis} offers a consolidated survey and activity chain level analysis for the remaining four metropolitan cities.
The table reaffirms our earlier finding that the Llama-2 base model closely approximates the actual data in both survey and activity chain level analyses compared to Gemini-pro and GPT-4.
However, the Llama-2 cannot handle travel time data accurately.
This deficiency is fixed when the Llama-2 model is trained on a limited number of samples, as evidenced by the simulated travel data of the \textit{Llama-2-trained-x-infer} model, which displays proper management of time-related data and shows the best performance, particularly in the weighted overlap of actual and simulated activity chains.

\begin{table}[h]
\begin{center}
\begin{tabular}{l|rrr}
\toprule
  & Avg. no &  Travel & Wt. overlap \\
  & of. locs &  time & of Actual\\
  & traveled &  (Hrs) & \& Simulated\\
\midrule 
\multicolumn{4}{c}{Washington-Arlington-Alexandria} \\
Actual &5.15 & 1.75 & - \\
Gemini-Pro &6.45 & 2.82 &  18.89 \\
GPT-4 &6.91 & 2.58 & 2.7\\
Llama-2 & 5.375 & 6.43 & 26.58\\
Llama-2-trained-x-infer & 4.68 & 1.56 & \textbf{40.15}\\
\midrule
\multicolumn{4}{c}{Los Angeles-Long Beach-Anaheim} \\
Actual &5.11 & 1.63 & - \\
Gemini-Pro &6.56 & 2.26 & 17.22 \\
GPT-4 & 6.88 & 2.53 & 1.51\\
Llama-2 & 5.63 & 6.22 & 27.29\\
Llama-2-trained-x-infer & 4.64 & 1.69 & \textbf{43.12}\\
\midrule
\multicolumn{4}{c}{Dallas-Fort Worth-Arlington} \\
Actual &5.14 & 1.52 & - \\
Gemini-Pro &6.31 & 2.31 & 18.4 \\
GPT-4 & 6.91 & 2.53 & 2.04\\
Llama-2 & 5.42 & 5.75 & 28.18\\
Llama-2-trained-x-infer & 4.68 & 1.56 & \textbf{44.42}\\
\midrule
\multicolumn{4}{c}{Minneapolis-St. Paul-Bloomington } \\
Actual & 5.10 & 1.61 & - \\
Gemini-Pro &6.24 & 2.42 & 16.99\\
GPT-4 & 7.10 & 2.54 & 2.27\\
Llama-2 & 5.73 & 6.59 & 24.44\\
Llama-2-trained-x-infer  & 4.75 & 1.44 & \textbf{45.84}\\
\bottomrule
\end{tabular}
\end{center}
\caption{Chain and activity level analysis for remaining cities reiterate that the trained model of Llama-2 demonstrates the closest resemblance to the actual survey data.}
\label{tab:inter_loc_travel_time_chain_analysis}
\end{table}

\begin{figure*}[ht]
    \centering
    \includegraphics[trim={1.3cm 0cm 1.2cm 1.3cm}, clip, width=\linewidth]{plots/norm2_inter_city.png}

    \caption{Forbenius norm between the first-order transition probabilities of actual and simulated surveys for different cities in various combinations for different LLMs.}
    \Description{Forbenius norm between the first-order transition probabilities of actual and simulated surveys for different cities in various combinations for different LLMs.}
    \label{fig:norm2_inter_city}
\end{figure*}

The trip level analysis across different cities yields interesting insights.
Figure~\ref{fig:norm2_inter_city} presents box plots illustrating the Forbenius norm between the first-order transition probabilities of actual and simulated surveys in various combinations for different LLMs.
The first plot compares the Forbenius norm between the first-order transition probabilities of actual and simulated surveys within the same city across different models.
Notably, the distribution of norms is lowest for  \textit{Llama-2-trained-x-infer}, indicating its proximity to the actual survey data.
The second plot displays the norms between actual and simulated surveys for different cities, revealing a comparable range of differences across all models as observed between actual and simulated surveys within the same cities, albeit with slightly greater variability.
This may seem counterintuitive, but the third plot sheds light on this phenomenon.
The third plot shows the norm among simulated surveys for different cities, along with that among actual surveys for different cities.
Here, we observe minimal differences among the first-order transition probabilities within both simulated and actual surveys across different cities.
This shows that a similar difference between the simulated and actual of different to that between the same cities is expected.
A holistic view of figure~\ref{fig:norm2_inter_city} underscores the superior performance of the \textit{Llama-2-x-infer} model in closely matching actual survey data. 
Additionally,  the similarity in differences between actual and simulated surveys across different cities, mirroring those within the same city, aligns with our finding that the difference among actual cities is also marginal.
This shows the overall effectiveness of our LLM-based travel survey simulation system.

With the transition probabilities, we also conduct ward hierarchical clustering~\cite{ward1963hierarchical} on both actual survey data and simulated surveys generated by different LLMs.
Cities are clustered into two groups.
The actual transition probabilities yielded two clusters: ``San Francisco-Oakland-Hayward, Los Angeles-Long Beach-Anaheim, and Washington-Arlington-Alexandria" and another ``Dallas-Fort Worth-Arlington and Minneapolis-St. Paul-Bloomington".
For the simulated data, the clustering that was closest to the actual one was observed with GPT-4 and \textit{Llama-2-trained-x-infer}, where Washington-Arlington-Alexandria shifted to the second cluster, resulting in two clusters: ``San Francisco-Oakland-Hayward and Los Angeles-Long Beach-Anaheim" and ``Dallas-Fort Worth-Arlington, Minneapolis-St. Paul-Bloomington, and Washington-Arlington-Alexandria."
This similarity of clusters, combined with Llama-2-trained-x-infers proximity to actual data, further validates the effectiveness of our LLM-based travel survey simulation system when utilizing Llama-2-trained models that are fine-tuned with a limited number of samples.

In conclusion, our LLM-based travel survey simulation system, particularly when paired with Llama-2 trained models, proves to be effective.
This is evident by its closest proximity to the actual surveys across survey, trip, and activity chain level analyses/
Furthermore, the clustering of transition probabilities for different cities yields similar cluster assignments, further affirming our system's efficacy.


% \begin{table}[h]
% \begin{center}
% \begin{tabular}{l|rrr}
% \toprule
%   &No. of.& Avg. no of. &  Travel \\
%   &Samples& locs traveled &  time (Hrs)\\
% \midrule 
% \multicolumn{4}{c}{Washington-Arlington-Alexandria} \\
% Actual & 1439 &5.15 & 1.75 \\
% Gemini-Pro & 1133 &6.45 & 2.82 \\
% Llama-2 & 1240 & 5.375 & 6.43 \\
% GPT-4 & 653 &6.91 & 2.58 \\
% Llama-2-trained-x-infer & 1210 & 4.68 & 1.56 \\
% \midrule
% \multicolumn{4}{c}{Los Angeles-Long Beach-Anaheim} \\
% Actual & 5534 &5.11 & 1.63 \\
% Gemini-Pro & 1299 &6.56 & 2.26 \\
% Llama-2 & 1225 & 5.63 & 6.22 \\
% GPT-4 & 683 & 6.88 & 2.53 \\
% Llama-2-trained-x-infer & 1213 & 4.64 & 1.69 \\
% \midrule
% \multicolumn{4}{c}{Dallas-Fort Worth-Arlington} \\
% Actual & 15977&5.14 & 1.52 \\
% Gemini-Pro & 1226 &6.31 & 2.31 \\
% Llama-2 & 1180 & 5.42 & 5.75 \\
% GPT-4 & 636 & 6.91 & 2.53 \\
% Llama-2-trained-x-infer & 1144 & 4.68 & 1.56 \\
% \midrule
% \multicolumn{4}{c}{Minneapolis-St. Paul-Bloomington } \\
% Actual & 1147 & 5.10 & 1.61 \\
% Gemini-Pro & 1293 &6.24 & 2.42 \\
% Llama-2 & 1181 & 5.73 & 6.59 \\
% GPT-4 & 662 & 7.10 & 2.54 \\
% Llama-2-trained-x-infer & 1148 & 4.75 & 1.44 \\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{Comparison of the average number of locations traveled and mean travel time across different models for remaining cities reiterate that the trained model of Llama-2 demonstrate the closest resemblance to the actual survey data.}
% \label{tab:inter_loc_travel_time}
% \end{table}


% \begin{table*}[ht]
% \begin{center}
% \begin{tabular}{l|rr|rr|rr|r}
% \toprule
%   & \multicolumn{2}{c}{Simulated in Actual} & \multicolumn{2}{c}{Simulated in  All Actual} & \multicolumn{2}{c}{Actual in Simulated} & Weight overlap of\\
%   & \% & Weight & \% & Weight &  \% & Weight & Actual and Simulated \\
% \midrule
% \multicolumn{8}{c}{Washington-Arlington-Alexandria} \\
% Gemini-Pro & 11.01 & 26.3 & 44.85 & 56.31 & 12.75 & 42.39 & 18.89  \\
% Llama-2 & 12.72 & 34.6 & 45.63 & 58.87 & 13.43 & 43.92 & 26.58\\
% GPT-4 & 4.4 & 4.29 & 42.75 & 56.81 & 2.31 & 4.59 & 2.7 \\
% Llama-2-trained-x-infer & \textbf{21.36} & \textbf{55.95} & \textbf{67.46} & \textbf{81.07} & \textbf{17.1} & \textbf{49.76} & \textbf{40.15} \\
% \midrule
% \multicolumn{8}{c}{Los Angeles-Long Beach-Anaheim} \\
% Gemini-Pro & 15.23 & 28.1 & 44.69 & 54.89 & 6.69 & 45.59 & 17.22  \\
% Llama-2 & 19.45 & 40.65 & 43.16 & 57.8 & 6.82 & 46.02 & 27.29\\
% GPT-4 & 7.3 & 8.78 & 37.78 & 49.63 & 1.28 & 1.81 & 1.51 \\
% Llama-2-trained-x-infer & \textbf{36.66} & \textbf{65.21} & \textbf{68.33} & \textbf{81.37} & \textbf{9.38} & \textbf{49.69} & \textbf{43.12} \\
% \midrule
% \multicolumn{8}{c}{Dallas-Fort Worth-Arlington} \\
% Gemini-Pro & 27.7 & 42.58 & 47.57 & 58.89 & 4.57 & 40.85 & 18.4  \\
% Llama-2 & 27.24 & 48.64 & 46.22 & 62.12 & 3.6 & 43.39 & 28.18\\
% GPT-4 & 16.1 & 22.17 & 42.44 & 53.46 & 1.2 & 3.03 & 2.04 \\
% Llama-2-trained-x-infer & \textbf{49.37} & \textbf{72.73} & \textbf{73.35} & \textbf{84.79} & \textbf{5.02} & \textbf{50.12} & \textbf{44.42} \\
% \midrule
% \multicolumn{8}{c}{Minneapolis-St. Paul-Bloomington} \\
% Gemini-Pro & 9.83 & 25.37 & 46.51 & 60.17 & 15.0 & 41.5 & 16.99  \\
% Llama-2 & 11.69 & 32.09 & 44.09 & 58.17 & 15.33 & 47.52 & 24.44\\
% GPT-4 & 3.06 & 3.47 & 41.07 & 53.63 & 2.0 & 3.49 & 2.27 \\
% Llama-2-trained-x-infer & \textbf{24.06} & \textbf{59.76} & \textbf{70.59} & \textbf{84.32} & \textbf{22.5} & \textbf{51.79} & \textbf{45.84} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{Activity chain analysis for the remaining cities reiterate that LLama-2 trained model best represent the actual travel chains with a high degree of correctness.}
% \label{tab:inter_chain_analysis}
% \end{table*}



==> sections/intra-city-results.tex <==
\section{Results of simulation for the San Francisco-Oakland-Hayward metropolitan area}
\label{sec:intra-city-results}

This section provides a detailed analysis of the outputs generated by our LLM-based travel survey simulation system for the San Francisco-Oakland-Hayward metropolitan area, comparing them to actual data from NHTS-2017 using the evaluation methodologies outlined in \S~\ref{sec:evaluation}.

\subsection{Survey level evaluation}
\begin{table}[h]
\begin{center}
\begin{tabular}{l|rrr}
\toprule
  &No. of.& Avg. no of. &  Travel \\
  &Samples& locs traveled ($\delta$) &  time (H)($\delta$)\\
\midrule
Actual & 4027&5.35 & 1.74 \\
\midrule
Gemini-Pro & 1241 &6.59 (1.24) & 2.52 (0.78) \\
GPT-4 & 688&6.96 (1.61) & 2.52 (0.78) \\
Llama-2 & 1279&5.55 (0.20) & 7.17 (5.43) \\
\midrule
Llama-2-trained & 1452&4.97 (-0.38) & 1.53 (-0.21) \\
Llama-2-trained-x-infer & 1435&4.79 (-0.56) & 1.60 (-0.14) \\
Llama-2-ens & 2714 &5.15 (-0.20) & 3.48 (1.74) \\
\bottomrule
\end{tabular}
\end{center}
% \caption{The average number of locations traveled and mean travel time for various models show that Llama-2 models trained variant are closest to actual survey when considering both the measures. }
\caption{Comparison of the average number of locations traveled and mean travel time across different models. The trained variants of Llama-2 demonstrate the closest resemblance to actual survey data.}
\label{tab:intra_loc_travel_time}
\end{table}

Table~\ref{tab:intra_loc_travel_time} presents the average number of locations traveled per survey along with the corresponding average travel times and sample sizes.
From the table, it is evident that among the base models, Llama-2 closely aligns with the actual number of locations traveled but falls short in terms of travel time accuracy.
This discrepancy can be attributed to differences in model alignment.
GPT-4 and Gemini-Pro are fine-tuned for better alignment with human instructions which makes them adept at handling numerical data or time data. 
In contrast, the base Llama-2 model lacks such fine-tuning that makes the model inept in handling numbers.
However, this alignment of GPT-4 and Gemini-Pro, while advantageous for travel time predictions, also leads to the generation of more text, consequently resulting in a higher number of locations traveled.
This trend is depicted in figure~\ref{fig:hist_intra_city}, which displays the distribution of the number of locations traveled by the survey respondents.
For Gemini-Pro and GPT-4, the number of locations traveled exceeds the actual data, particularly for longer journeys.
This issue is exacerbated for GPT-4 which shows limited variability in the number of locations traveled.
Conversely, the distribution for Llama-2 base models and its trained variants is more evenly distributed and closely aligns with the actual distribution.

\begin{figure}[ht]
    \centering
    \includegraphics[trim={1.3cm 1.3cm 1.2cm 1.2cm}, clip, width=\linewidth]{plots/hist_intra_city.png}

    \caption{Distribution of the number of locations traveled by survey respondents for the San Francisco-Oakland-Hayward metropolitan area for different LLMs compared to the actual survey shows that Llama-2 and its trained variants are better aligned with the actual data.}
    \Description{Distribution of the number of locations traveled by survey respondents for the San Francisco-Oakland-Hayward metropolitan area for different LLMs compared to the actual survey shows that Llama-2 and its trained variants are better aligned with the actual data.}
    \label{fig:hist_intra_city}
\end{figure}
The limitation of the llama-2 base model in handling numerical data, and consequently travel time is evident in figure~\ref{fig:tt_intra_city}, where we present the travel times of each model in a box plot.
We can see from the figure that the travel time for llama-2 is as high as 120 hours in a survey of 24 hours, indicating its struggle with time-related data.
Conversely, Gemini-pro and GPT-4 base models demonstrate closer alignment with actual travel times.
This ineptitude of llama-2 in handling time-related data is addressed by the trained Llama models, as seen in figure~\ref{fig:tt_intra_city}, where both trained variants exhibit closer proximity to actual travel times.
\begin{figure}[ht]
    \centering
    \includegraphics[trim={1.2cm 1.2cm 1.2cm 1.2cm}, clip, width=\linewidth]{plots/tt_intra_city.png}
    \caption{Travel time predictions reveal that Gemini-Pro and GPT-4 models outperform Llama-2, while the trained Llama-2 models achieve similar accuracy. The left plot is the full box plot and the right one excludes outliers.}
    \Description{Travel time predictions reveal that Gemini-Pro and GPT-4 models outperform Llama-2, while the trained Llama-2 models achieve similar accuracy.}
    \label{fig:tt_intra_city}
\end{figure}

Overall, the survey-level evaluation across various models indicates that Llama-2-based simulated travel survey data, specifically the trained llama-2 variants, show the highest fidelity to the actual travel survey data.

\subsection{Trip level evaluation}

\begin{table}[h]
\begin{center}
\begin{tabular}{l|rr}
\toprule
  & \multicolumn{2}{c}{Frobenius Norm with} \\
  & 1st order&  2nd order\\
  &transition prob &transition prob \\
\midrule
Gemini-Pro & 0.063 & 0.046 \\
GPT-4 & 0.166 & 0.130 \\
Llama-2 & 0.106 & 0.071 \\
\midrule
Llama-2-trained & 0.044 & \textbf{0.0319} \\
Llama-2-trained-x-infer & \textbf{0.043} & 0.036 \\
Llama-2-ens & 0.068 & 0.047 \\
\bottomrule
\end{tabular}
\end{center}
% "Frobenius Norm comparison of transition probabilities demonstrates the closest resemblance between Llama-2 trained variants and actual survey data."
\caption{Frobenius Norm comparison of transition probabilities shows the closest resemblance between Llama-2 trained variants simulated data and actual survey data.}
\label{tab:intra_norm2}
\end{table}

Table~\ref{tab:intra_norm2} presents the Forbenius norm of transition probabilities, comparing simulated travel survey data generated by different LLMs against the actual travel survey data.
The results indicate that the trained variants of Llama-2 show the closest resemblance to the actual transition probabilities.
Specifically, \textit{Llama-2-trained-x-infer}, which excludes the test city of the San Francisco-Oakland-Hayward metropolitan area from its training dataset, shows the closest alignment in terms of first-order transition probabilities, while \textit{Llama-2-trained-x-infer}, which includes the test city in its training dataset, is closest in terms of second-order transition probabilities.
Despite minor variations, both models demonstrate comparable performance, suggesting the efficacy of training even in the absence of location-specific data.
Among the base models, Gemini-Pro shows the closest resemblance, with GPT-4 performing poorly.

\begin{figure}[ht]
    \centering
    \includegraphics[trim={1.2cm 1.25cm 1.2cm 1.27cm}, clip, width=\linewidth]{plots/dest_prob_intra_city.png}

    \caption{Difference in first order destination probabilities (original - generated).}
    \Description{Difference in first order destination probabilities (original - generated).}
    \label{fig:dest_prob_intra_city}
\end{figure}

This variation in model performance can be explained with the help of figure~\ref{fig:dest_prob_intra_city}, which illustrates the difference in the first-order destination probabilities between the actual survey and simulated survey ordered by their probabilities in the actual survey. 
The first-order destination probabilities are computed based on the first-order transition probabilities, where we consider solely the likelihood of a trip ending at a particular location type.
The figure illustrates the alignment issue discussed in the preceding sub-section.
Specifically, it demonstrates that Gemini-Pro and GPT-4 models tend to over-predict destinations typically associated with tasks such as shopping, dining out, or recreational activities, reflecting the fact that they have been fine-tuned or aligned to respond to similar kinds of queries.
While Llama-2 also exhibits similar tendencies of over-predicting location types, particularly if we consider work location type, which Llama-2 overpredicts by 100 percent, it generally is closest to the actual survey.
Moreover, the trained variants of Llama-2 demonstrate destination probabilities most similar to the actual data, albeit with a slight deviation.
Our aim here is not an exact match but rather a destination probability within a small percentage range of actual probabilities, criteria met by the trained Llama-2 models.
The analysis of second-order destination probabilities also shows a similar trend, as illustrated in Figure~\ref{fig:dest_prob_2_intra_city} in Appendix~\ref{sec_c:supporting_figures}.

In summary, the trip-level evaluation across various models indicates that Llama-2-trained-based simulated travel survey data show the highest fidelity to the actual travel survey data, which aligns with our survey-level evaluation.

\subsection{Activity chain level evaluation}



\begin{table*}[ht]
\begin{center}
\begin{tabular}{l|rr|rr|rr|r}
\toprule
  & \multicolumn{2}{c}{Simulated in Actual} & \multicolumn{2}{c}{Simulated in  All Actual} & \multicolumn{2}{c}{Actual in Simulated} & Weight overlap of\\
  & \% & Weight & \% & Weight &  \% & Weight & Actual and Simulated \\
\midrule
Gemini-Pro & 15.55 & 29.81 & 46.22 & 56.79 & 7.77 & 39.21 & 17.25  \\
GPT-4 & 7.89 & 11.92 & 40.71 & 52.76 & 1.63 & 2.19 & 1.44 \\
Llama-2 & 15.54 & 36.12 & 43.06 & 57.39 & 6.88 & 39.14 & 25.42\\
\midrule
Llama-2-trained & \textbf{30.88} & 61.16 & 65.44 & 80.1 & 11.92 & 48.22 & \textbf{42.54} \\
Llama-2-trained-x-infer & 30.04 & \textbf{61.88} & \textbf{67.24} & \textbf{81.39} & 11.02 & 46.49 & 40.9 \\
Llama-2-ens & 18.97 & 49.74 & 51.96 & 70.08 & \textbf{14.49} & \textbf{51.6} & 40.16 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Activity chain analysis for the San Francisco-Oakland-Hayward metropolitan area shows that LLama-2 trained variants best represent the actual travel chains with a high degree of correctness.}
\label{tab:intra_chain_analysis}
\end{table*}

Table~\ref{tab:intra_chain_analysis} presents a comprehensive overview of our activity chain level evaluation results for the San Francisco-Oakland-Hayward metropolitan area.
The table structure is as follows: the first column denotes the models, followed by two columns of the simulated activity chains present in the actual activity chains of the San Francisco-Oakland-Hayward metropolitan area and the actual activity chains of all the cities in the NHTS-2017 survey, denoted as `Simulated in Actual' and `Simulated in All Actual' respectively. 
The fourth column, labeled `Actual in Simulated', represents the actual activity chains that are present in the simulated activity chains.
Each of the second, third, and fourth columns is subdivided into percentage and weight columns, delineating the proportion of unique activity chains (\%) and their contribution to the overall chains (weight).
The final column, titled `Weight overlap of Actual and Simulated', depicts the weighted overlap between the actual and simulated activity chains. 
The `Simulated in Actual' column represents the proximity of simulated activity chains to the actual chains of the specific city.
On the other hand `Simulated in All Actual' column acts as a measure of the correctness of simulated activity chains because if these chains are found in activity chains in any other cities as well, they are considered correct.
The `Actual in Simulated' column reflects the representativeness of the simulated activity chains by showcasing the portion of the actual activity chains present within them.
Finally, the last column provides an exact overlap of the activity chains along with their weights,  serving as a consolidated measure of consistency between the actual and simulated travel chains.

From table~\ref{tab:intra_chain_analysis}, it is evident that the llama-2 trained variants outperform other models across the different activity chain analyses.
Llama-2 trained variants exhibit approximately 60 percent of their activity chains by weight present in the actual travel chains, compared to around 36 percent for the base llama and progressively lower for Gemini-pro and GPT-4.
This indicates that the simulated activity chains from the Llama-2 trained variants are close to actual activity chains.
Moreover, Llama-2 trained variants encompass around 81 percent by weight, or 67 percent uniquely, of activity chains in the overall NHTS-2017 survey activity chains, signifying their superior accuracy compared to the base Llama-2, Gemini-pro, and GPT-4, which fall within the range of 50 percent correctness.
Additionally, we also assessed the correctness of unmatched activity chains from the \textit{Llama-2-trained-x-infer} using the Levenshtein distance~\cite{yujian2007normalized}.
We found that among the remaining unmatched chains, \textbf{\(68.50\)} percent have an edit distance of \(1\), \textbf{\(22.44\)} percent have an edit distance of \(2\), \textbf{\(6.29\)} percent have an edit distance of \(4\), and the remaining \textbf{\(2.75\)} percent have a higher edit distance, further validating the correctness of the unmated portion of the simulated activity chains.
Further, approximately 47 percent by weight of actual activity chains are present in the simulated activity chains of the Llama-2 trained variants, compared to around 39 percent for the Llama-2 base model and Gemini-pro, and only 2 percent for GPT-4.
This demonstrates that the Llama-2 trained variants most accurately represent activity chains observed in the actual survey.
Finally, the weighted overlap between the actual and simulated activity chains surpasses 41 percent for the Llama-2 trained variants, exceeding Gemini-pro by more than 20 percent and GPT-4 by 40 percent, which further solidifies the superiority of Llama-2 trained models at representing the activity chains present in the actual survey.

\begin{figure}[ht]
    \centering
    \includegraphics[trim={1.33cm 1.33cm 1.43cm 1.25cm}, clip, width=\linewidth]{plots/chains_intra_city.png}

    \caption{The cumulative sum of activity chain counts for the San Francisco-Oakland-Hayward metropolitan area's actual survey, compared with those from various LLM-based simulations, indicates that Llama-2 trained variants closely mirror the actual survey. }
    \Description{The cumulative sum of activity chain counts for the San Francisco-Oakland-Hayward metropolitan area's actual survey, compared with those from various LLM-based simulations, indicates that Llama-2 trained variants closely mirror the actual survey. .}
    \label{fig:chains_intra_city}
\end{figure}

This superiority of Llama-2 trained models in accurately representing the activity chains present in the actual survey is further clarified in figure~\ref{fig:chains_intra_city}, where the cumulative sum of the activity chains counts is plotted in comparison to matched activity chains counts across various models.
Additionally, activity chains for the Los Angeles-Long Beach-Anaheim metropolitan area are also plotted for better comparison.
Vertical lines indicating the start of activity chains with less than 10 counts and those with only 1 count are also in the plot, which depicts the sparsity of activity chains.
The figure illustrates that GPT-4 exhibits the least resemblance, followed by Gemini-pro and then the Llama-2 base model.
Conversely, the Llama-2 trained models closely match the actual chains, akin to how the activity chains of the Los Angeles-Long Beach-Anaheim metropolitan area match the San Francisco-Oakland-Hayward metropolitan area.
This result is particularly intriguing, as we will see in the next sections that the difference between the travel surveys of different cities is very nominal,
suggesting a noteworthy level of simulation accuracy.
We have also plotted the distribution of the top hundred activity chains by the count of the actual survey in comparison to other simulated surveys in Figure~\ref{fig:chain_hist_intra_city} in Appendix~\ref{sec_c:supporting_figures} which further illustrates our argument.

Overall, the survey, trip, and activity chain level evaluation across various models indicate that Llama-2-trained-based simulated travel survey data show the highest fidelity to the actual travel survey data.

==> sections/problem_statement.tex <==
\section{Problem Statement}
\label{sec:problem_statement}

==> sections/results.tex <==
\section{Results}


\begin{table*}[]
\begin{center}
\begin{tabular}{l|rrrr|rrrr|rrrr}
\toprule
  % & \multicolumn{4}{c}{\bf No. of} &4&3&2&1 \\
  % & \multicolumn{6}{c}{\bf No. of} &  \multicolumn{3}{c}{} \\
\multicolumn{1}{c}{\bf }  &\multicolumn{4}{c}{\bf No. Samples} &\multicolumn{4}{c}{\bf No. Locations}&\multicolumn{4}{c}{\bf Travel time (Hrs)}\\

  & A & Gemini & Llama2 & GPT-4 & A & Gemini & Llama2 & GPT-4 & A & Gemini & Llama2 & GPT-4 \\
\midrule
SF& 4027 & 1241 & 1279 & 688 & 5.35 & 6.60 & 5.56 & 6.96 & 1.74 & 2.53 & 7.18 & 2.52  \\
DC& 1439 & 1133 & 1240 & 653 & 5.15 & 6.45 & 5.38 & 6.91 & 1.75 & 2.82 & 6.43 & 2.58 \\
DFW& 15977 & 1226 & 1180 & 636 & 5.14 & 6.31 & 5.43 & 6.91 & 1.52 & 2.31 & 5.76 & 2.58  \\
LA& 5534 & 1299 & 1225 & 683 &5.12 & 6.57 & 5.64 & 6.88 & 1.64 & 2.26 & 6.23 & 2.53  \\
Minneapolis& 1147 & 1293 & 1181 & 662 & 5.10 & 6.24 & 5.73 & 7.10 & 1.62 & 2.42 & 6.59 & 2.54  \\
\bottomrule
\end{tabular}
\end{center}
\caption{The number of locations traveled and travel time. * denotes statistical significance between the values (No statistical significance was found). }
\label{tab:inter_locs}
\end{table*}


\begin{table}[H]
\begin{center}
\begin{tabular}{l|rrr|rrr}
\toprule
\multicolumn{1}{c}{\bf }  &\multicolumn{3}{c}{\bf Overlap } &\multicolumn{3}{c}{\bf Exact Overlap}\\

  & Gemini & Llama2 & GPT-4 & Gemini & Llama2 & GPT4 \\
\midrule
SF & 39.21 & 39.13 & 2.18 & 17.25 & 25.41 & 1.43  \\
DC & 42.39 & 43.91 & 4.58 & 18.89 & 26.58 & 2.69  \\
DFW & 40.84 & 43.39 & 3.03 & 18.39 & 28.14 & 2.04  \\
LA & 45.59 & 46.02 & 1.81 & 17.21 & 27.29 & 1.51  \\
Minneapolis& 41.50 & 47.52 & 3.49 & 16.99 & 24.43 & 2.27  \\
\bottomrule
\end{tabular}
\end{center}
\caption{Activity chains present in the original data}
\label{tab:inter_overlap}
\end{table}


\begin{table}[H]
\begin{center}
\begin{tabular}{l|rrr}
\toprule
\multicolumn{1}{c}{\bf }  &\multicolumn{3}{c}{\bf Pearson Correlation } \\

  & Gemini & Llama2 & GPT-4  \\
\midrule
SF & 0.65 & 0.86 & -0.08 \\
DC & 0.69 & 0.88 & 0.38 \\
DFW & 0.61 & 0.88 & 0.07 \\
LA & 0.65 & 0.85 & 0.25 \\
Minneapolis& 0.66 & 0.84 & 0.42 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Pearson Correlation Coefficient between the count of activity chains with the actual data}
\label{tab:inter_corr}
\end{table}
